Compositional Score Modeling for Simulation-based Inference

Neural Posterior Estimation methods for simulation-based inference can be ill-suited for dealing with posterior distributions obtained by conditioning on multiple observations, as they tend to require a large number of simulator calls to learn accurate approximations. In contrast, Neural Likelihood Estimation methods can handle multiple observations at inference time after learning from individual observations, but they rely on standard inference methods, such as MCMC or variational inference, which come with certain performance drawbacks. We introduce a new method based on conditional score modeling that enjoys the benefits of both approaches. We model the scores of the (diffused) posterior distributions induced by individual observations, and introduce a way of combining the learned scores to approximately sample from the target posterior distribution. Our approach is sample-efficient, can naturally aggregate multiple observations at inference time, and avoids the drawbacks of standard inference methods.

==> fnspe_nspe.tex <==
% \section{Score Modeling for SBI} \label{sec:ndpe}

% % This section presents our approach for SBI. As mentioned in \cref{sec:intro} our goal is to develop a method that (i) can naturally aggregate an arbitrary number of observations at inference time while requiring a low number of simulator calls per training sample; and (ii) avoids the limitations of generic inference methods. We achieve this by building on conditional score modeling, but using a different construction for the bridging densities and reference distribution to the ones typically used. \Cref{sec:ndpe_sub} presents our approach, and \cref{sec:diff_npe} explains why a direct application of conditional score-based methods (as described in \cref{sec:sbgm}), called Neural Score Posterior Estimation (\nspe), fails to satisfy (i) and (ii). Finally, \cref{sec:pndpe} presents Partially Factorized Neural Score Posterior Estimation (\pfnspe), a family of methods that generalizes \fnspe and \nspe and smoothly interpolates between them.

% This section presents \fnspe, our approach to SBI. Our goal is to develop a method that (i) can aggregate an arbitrary number of observations at inference time while requiring a low number of simulator calls per training sample; and (ii) avoids the limitations of generic inference methods. We achieve this by building on conditional score modeling, but using a different construction for the bridging densities and reference distribution to the ones typically used. \Cref{sec:ndpe_sub} presents our approach, and \cref{sec:diff_npe} explains why this novel construction is necessary, by showing that \nspe, the direct application of the score modeling framework to the SBI task, fails to satisfy (i). Finally, \cref{sec:pndpe} presents \pfnspe, a family of methods that generalizes \fnspe and \nspe by smoothly interpolating between them.

% \subsection{Factorized Neural Posterior Score Estimation} \label{sec:ndpe_sub}

% \fnspe builds on the conditional score modeling framework, but with a different construction for the bridging densities and reference distribution. Our construction is based on the  factorization of the posterior in terms of the posteriors induced by individual observations (see \cref{app:derfact}):
% \begin{equation} \label{eq:postfact}
% p(\theta \vert x_{1}, \ldots, x_{n}) \propto p(\theta)^{1-n} \prod_{j=1}^n p(\theta \vert x_{j}).
% \end{equation}
% The main idea behind our approach is to define bridging densities that satisfy a similar factorization. To achieve this we propose the sequence indexed by $t=0, \ldots, T$ given by
% \begin{equation} \label{eq:approachbr}
%     \ptf(\theta \vert x_1, \hdots, x_n) \propto \left(p(\theta)^{1-n}\right)^{\frac{T-t}{T}} \prod_{j=1}^n p_t(\theta \vert x_{j}),
% \end{equation}
% where $p_t(\theta \vert x_{j})$ follows \cref{eq:sbmbr} with $c=x_j$, and the super-script \textit{f} is used as an identifier of \fnspe.

% This construction has four key properties. First, the distribution for $t=0$ recovers the target $p(\theta \vert x_{1}, \ldots, x_{n})$. Second, the distribution for $t=T$ approximates a spherical Gaussian $\pTf(\theta \vert x_1, \hdots, x_n) \approx p_T(\theta) = \mathcal{N}(\theta\vert 0, \frac{1}{n} I)$, since the prior term vanishes and  $p_T(\theta \vert x_j) \approx \mathcal{N}(\theta\vert 0, I)$, and thus can be used as a tractable reference for the process. Third, the scores of the resulting densities can be decomposed in terms of the score of the prior (typically available exactly) and the scores of the individual $p_t(\theta \vert x_j)$ terms as 
% \begin{multline}
%     \nt \log \ptf(\theta \vert x_1, \hdots, x_n) = \\ \frac{(1-n)(T-t)}{T} \nt \log p(\theta) + \sum_{j=1}^n \nt \log p_t(\theta \vert x_{j}).
% \end{multline}
% And fourth, the scores $\nt \log p_t(\theta \vert x_{j})$ can all be approximated using a \textit{single} score network $s_\psi(\theta, t, x)$ trained via denoising score matching using samples $(\theta^i, x^i) \sim p(\theta) p(x\vert \theta)$, as explained in \cref{sec:sbgm}.

% After training, given i.i.d.\ observations $x^o_1, \hdots, x^o_n$, we can approximately sample $p(\theta \vert x^o_1, \hdots, x^o_n)$ by running \cref{alg:sampleuld} with the reference $p_T(\theta) = \mathcal{N}(\theta\vert 0, \frac{1}{n} I)$, conditioning variable $c = \{x^o_1, \hdots, x^o_n\}$, and approximate score
% \begin{multline} \label{eq:scoreapprox}
%     s_\psi(\theta, t, c) = \\ \frac{(1-n)(T-t)}{T} \nt \log p(\theta) + \sum_{j=1}^n s_\psi(\theta, t, x^o_j).
% \end{multline}

% In short, the fact that the bridging densities factorize in terms of each individual observation as in \cref{eq:approachbr} allows us to train a score network to approximate the scores of the distributions induced by individual observations, and to aggregate the network's output for different observations at inference time to sample the target posterior distribution. Therefore, this approach can aggregate an arbitrary number of observations at inference time while training on samples $(\theta^i, x^i)\sim p(\theta) p(x\vert \theta)$, each one requiring a single simulator call. Additionally, the mass-covering properties of score-based methods \cite{ho2020denoising, song2021maximum} together with the annealed sampling algorithm avoid the drawbacks of standard inference methods, such as their difficulty in handling multi-modality.

% % This approach satisfies our original desiderata: (i) it can naturally handle \textit{any} number of observations at inference time while training on samples $(\theta^i, x^i)\sim p(\theta) p(x\vert \theta)$ that require a single simulator call; and (ii) the mass-covering properties of score-based methods \cite{ho2020denoising, song2021maximum} together with the annealed sampling algorithm avoids the mode-seeking behavior of generic inference methods.

% % This approach satisfies our original desiderata: (i) it can naturally handle \textit{any} number of observations at inference time, as it relies on annealed Langevin dynamics with \cref{eq:scoreapprox}, which can be used with any $n$; (ii) the score network $s_\psi(\theta, t, x)$ is trained using samples $(\theta^i, x^i)\sim p(\theta) p(x\vert \theta)$, each one requiring a single simulator call, regardless of the number of conditioning variables at inference time; and (iii) the mass-covering properties of score-based methods \cite{ho2020denoising, song2021maximum} together with the annealed sampling algorithm avoids the mode-seeking behavior of generic inference methods.

% One potential drawback of \fnspe is that it might accumulate errors when combining score estimates as in \cref{eq:scoreapprox}, affecting the method's performance. This drawback is shared by all \nle and \nre methods, and we study it in empirically in \cref{sec:exps}.


% \subsection{Direct application of conditional score modeling} \label{sec:diff_npe}

% This section introduces \nspe and explains why it fails to satisfy our desiderata, specifically (i). \nspe consists on a direct application of the score modeling framework from \cref{sec:sbgm} to the SBI task. Following \cref{eq:sbmbr} with $c = \{x_1, \ldots, x_n\}$, and assuming a fixed number of observations $n$ (relaxed later), \nspe defines the sequence of densities
% % \begin{align} \label{eq:score_naive}
% %     p_0(\theta \vert x_1, \hdots, x_n) & = p(\theta \vert x_1, \hdots, x_n)\\
% %     p_t(\theta \vert x_1, \hdots, x_n) & = \int d\theta' \, p(\theta'\vert x_1, \hdots, x_n) p_t(\theta\vert \theta'), \nonumber
% % \end{align}
% \begin{equation} \label{eq:score_naive}
%     p_t(\theta \vert x_1, \hdots, x_n) = \int d\theta' \, p(\theta'\vert x_1, \hdots, x_n) p_t(\theta\vert \theta'),
% \end{equation}
% and trains a score network $s_\psi(\theta, t, x_1, \ldots, x_n)$ to approximate their scores via denoising score matching. Then, at inference time, given observations $x_1^o,\ldots,x_n^o$, \nspe uses $s_\psi(\theta, t, x^o_1, \ldots, x^o_n)$ to approximately sample $p(\theta \vert x_1^o, \ldots, x_1^o)$. \nspe can be extended to cases where $n$ is not fixed a priori, by parameterizing the score network as $s_\psi(\theta, t, x_1, \ldots, x_n) = s_\psi(\theta, t, h_\psi(x_1, \ldots, x_n), n)$ with a permutation-invariant function $h_\psi$, and training it with samples $(n^i, \theta^i, x_1^i, \ldots, x_n^i) \sim \mathcal{U}(n;n_{\max}) p(\theta) \prod_{i=1}^n p(x_i \vert \theta)$, where $\mathcal{U}(\cdot ;n_{\max})$ is the uniform distribution over $\{1, \ldots, n_{\max}\}$.

% Unfortunately, \nspe does not satisfy condition (i) outlined above, as it requires specifying the maximum number of observations $n_{\max}$ and needs $n_{\max} / 2$ simulator calls per training sample on average. Since the scores of the bridging densities defined in \cref{eq:score_naive} do not factorize in terms of the individual observations, the approach taken by \fnspe, which trains a score network for individual observations and aggregates them at inference time, is not applicable. However, in contrast to \fnspe, \nspe does not require adding approximations, so it does not accumulate errors.

% % To the best of our knowledge, \nspe has not been proposed before (it has been concurrently proposed by \citet{sharrock2022sequential}). However, since the method can be seen as a direct modification of \npe, replacing the conditional density estimator by a conditional diffusion model, we consider this to be a minor contribution of this work. \tg{Remove this?} \am{Yes.}

% % We now show that a direct application of conditional score modeling (presented in \cref{sec:sbgm}) to the SBI task fails to satisfy our desiderata, specifically (i) and (ii). Essentially, this is because the bridging densities defined do not factorize in terms of individual observations. Thus, the score network must be trained to handle multiple observations using inefficient samples. Following \cref{eq:sbmbr} with $c = \{x_1, \ldots, x_n\}$, and assuming a fixed number of observations $n$ (relaxed later), conditional score-based methods define the sequence of densities \tgf{Should we use different names for the sequence of densities used by each method? Right now we are calling all of them $p_t$, which may be confusing}
% % \begin{align} \label{eq:score_naive}
% %     p_0(\theta \vert x_1, \hdots, x_n) & = p(\theta \vert x_1, \hdots, x_n)\\
% %     p_t(\theta \vert x_1, \hdots, x_n) & = \int d\theta' \, p(\theta'\vert x_1, \hdots, x_n) p_t(\theta\vert \theta'), \nonumber
% % \end{align}
% % and train a score network $s_\psi(\theta, t, x_1, \ldots, x_n)$ to approximate their scores via denoising score matching. Then, at inference time, given observations $x_1^o,\ldots,x_n^o$, these methods use $s_\psi(\theta, t, x^o_1, \ldots, x^o_n)$ to approximately sample $p(\theta \vert x_1^o, \ldots, x_1^o)$. We call this approach Neural Score Posterior Estimation (\nspe).\footnote{We use this name for consistency with concurrent work by \citet{sharrock2022sequential} that explores this method, albeit for $n=1$.}
% % The method can be seen as a straightforward modification of \npe methods, replacing the conditional flow by a conditional diffusion model. Therefore, similarly to \npe, it can be adapted to scenarios where $n$ is not fixed a priori, by defining the score network as $s_\psi(\theta, t, x_1, \ldots, x_n) = s_\psi(\theta, t, h_\psi(x_1, \ldots, x_n), n)$ with a permutation-invariant function $h_\psi$, and training it using samples $(n^i, \theta^i, x_1^i, \ldots, x_n^i) \sim \mathcal{U}(n;n_{\max}) p(\theta) \prod_{i=1}^n p(x_i \vert \theta)$, where $\mathcal{U}(\cdot ;n_{\max})$ is the uniform distribution over $\{1, \ldots, n_{\max}\}$.

% % Unfortunately, \nspe does not satisfy conditions (i) and (ii) outlined above. This is because the scores of the bridging densities defined in \cref{eq:score_naive} do not factorize in terms of the individual observations $x_i$. Therefore, the approach taken by \fnspe, which trains a score network for individual observations and combines the approximations at inference time, is not applicable. \nspe requires, on average, $n_{\max}/2$ simulator calls per training sample. However, in contrast to \fnspe, the method does not require adding approximate terms, so it does not accumulate errors.

% \subsection{Partially Factorized Neural Posterior Score Estimation} \label{sec:pndpe}

% We introduced \nspe and \fnspe, and described their benefits and limitations. Namely, the latter is efficient in terms of number of simulator calls but may accumulate errors, while the opposite is true for the former. We now argue that these two approaches can be seen as the opposite extremes of a family of methods that interpolate between them, achieving different trade-offs between sample efficiency and accumulation of errors. We call these methods Partially Factorized Neural Posterior Score Estimation (\pfnspe).

% \pfnspe is based on a similar strategy to the one used by \fnspe, but using small subsets of observations instead of individual observations to factorize the target posterior distribution. Specifically, given $m\geq 1$, we partition the set of conditioning variables $\{x_1, \ldots, x_n\}$ into $k=\ceil{n/m}$ disjoint subsets of size at most $m$, denoted by $X_{1}, \ldots, X_{k}$, and factorize the posterior distribution as
% \begin{equation} \label{eq:partialpostfact}
% p(\theta \vert x_{1}, \ldots, x_{n}) \propto p(\theta)^{1-k} \prod_{j=1}^k p(\theta \vert X_{j}).
% \end{equation}
% Then, following the \fnspe strategy, we define the bridging densities using the diffused versions of each $p(\theta \vert X_{j})$ as 
% \begin{equation} \label{eq:parttialapproachbr}
%     \ptpf(\theta \vert x_1, \hdots, x_n) \propto \left(p(\theta)^{1-k}\right)^{\frac{T-t}{T}} \prod_{j=1}^k p_t(\theta \vert X_{j}),
% \end{equation}
% and train a score network $s_\psi(\theta, t, X_j)$ to approximate their scores. Since this network must handle as input sets $X_j$ of sizes varying between $1$ and $m$, we parameterize it using a permutation-invariant function, and train it using samples with a varying number of observations between $1$ and $m$, $(n, \theta, x_1, \ldots, x_n) \sim \mathcal{U}(n;m) p(\theta) \prod_{i=1}^n p(x_i\vert \theta)$.
% % \am{This is probably suboptimal, since we care more about good performance for $n=m$ than for other values of $m$.} \tg{Yes, as we do it now this is true. Should we comment on this?}

% At inference time, given observations $x_1^o,\ldots,x_n^o$, the method approximately samples the target $p(\theta \vert x^o_1, \ldots, x^o_n)$ by partitioning the observations into subsets $X^o_1,\ldots,X^o_k$ and running annealed Langevin dynamics (\cref{alg:sampleuld}) with $c = \{X^o_1, \hdots, X^o_{k}\}$ and the approximate score
% \begin{multline} \label{eq:partialscoreapprox}
%     s_\psi(\theta, t, c) = \\ \frac{(1-n)(T-t)}{T} \nt \log p(\theta) + \sum_{j=1}^k s_\psi(\theta, t, X^o_j).
% \end{multline}

% The value of $m$ controls the trade-off between sample efficiency and error accumulation: for a given $m$, the method gets an approximate score by adding $k=\ceil{n/m}$ terms (\cref{eq:partialscoreapprox}), and requires on average $m/2$ simulator calls per training sample. Therefore, low values of $m$ yield methods closer to \fnspe, while larger values yield methods closer to \nspe. In fact, we recover \fnspe for $m=1$  and \nspe for $m=n_{\max}$. This motivates finding the value of $m$ that achieves the best trade-off. We investigate this empirically in \cref{sec:exps}, where we observe that using low values of $m$ (but greater than 1) often yields the best results.

